Pareto Optimal Algorithmic Recourse in Multi-cost Function

In decision-making systems, algorithmic recourse aims to identify minimal-cost actions to alter an individual features, thereby obtaining a desired outcome. This empowers individuals to understand, question, or alter decisions that negatively affect them. However, due to the variety and sensitivity of system environments and individual personalities, quantifying the cost of a single function is nearly impossible while considering multiple criteria situations. Most current recourse mechanisms use gradient-based methods that assume cost functions are differentiable, often not applicable in real-world scenarios, resulting in sub-optimal solutions that compromise various criteria. These solutions are typically intractable and lack rigorous theoretical foundations, raising concerns regarding interpretability, reliability, and transparency from the explainable AI (XAI) perspective. To address these issues, this work proposes an algorithmic recourse framework that handles non-differentiable and discrete multi-cost functions. By formulating recourse as a multi-objective optimization problem and assigning weights to different criteria based on their importance, our method identifies Pareto optimal recourse recommendations. To demonstrate scalability, we incorporate the concept of epsilon-net, proving the ability to find approximated Pareto optimal actions. Experiments show the trade-off between different criteria and the methods scalability in large graphs. Compared to current heuristic practices, our approach provides a stronger theoretical foundation and better aligns recourse suggestions with real-world requirements.

==> algorithm/analyze.tex <==

\textbf{time complexity}

When we run the dynamic programming equation (1) in multi-shortest path algorithm. The time complexity analysis involves two main steps: concatenate and prune, which are repeated for at most $V-1$ iterations based on the Bellman-Ford algorithm for all edges. In the concatenate step, for each vertex v, we combine the distance tables $D_{u \in in(v)}$ from all incoming neighbors u $\in$ in(v) with the respective edge costs $d(u, v)$. This step has a time complexity of $O(n)$, where n is the size of the distance table $D$.

The subsequent pruning step aims to retain only the optimal solutions in the concatenated distance table. The time complexity of this pruning operation depends on the number of criteria considered. When dealing with two criteria, the pruning step leverages the theory of maximal point sets, resulting in a time complexity of O(n). However, when the number of criteria exceeds two, the time complexity increases to $O(n\log^{n-3}\log\log n)$.

Considering both the concatenate and prune steps, the overall time complexity of the multi-shortest path algorithm is $O(n|V||E|)$. Here, $|V|$ and$ |E|$ represent the number of vertices and edges in the graph respectively. The factor n accounts for the size of the distance table $D$, which may vary depending on the specific problem instance and the number of criteria considered.

 \textbf{correctness}
% we need to prove two things:\\

% \begin{itemize}
   
%      \item [(1)]
%     All optimal solution are in $D$
%      \item [(2)]
%     All solution in $D$ is optimal (when without constraint for $D$ size)
% \end{itemize}
% once we can prove (1) and (2) are correct, which means (1) equals to (2),then we can prove our algorithm is correct. Here is the prove for item 1, since the dp equation has already consider all edge that link in to $v$, we can promised that we find all possible temporary solution, which containing all optimal solutions.
% As for item 2, Assume $f(v,\ell)$ is Pareto optimal and $\exists$ $d_u \in f(u, \ell-1)$ is not Pareto optimal solution. Since the feature of Monotonicity of cost function. After $d_u \in f(u, \ell-1)$ connect with weight cost$ \overline{uv} $ still is not Pareto optimal solution. After step of prune, those worse solution would be dominate, which means $f(v,\ell)$ will not be the Pareto optimal solution. $\to \gets .$ Q.E.D. that, $\forall d_v \in f(v, \ell)$ is Pareto optimal, then $\forall _{u \in \text{in}(v)} \left(f(u, \ell - 1) + d(u, v)\right) and \forall d_v \in f(v, \ell - 1)$ must be Pareto optimal solution. To be more specific, only when last iteration are Pareto optimal, can next iteration still contain all Pareto optimal solution. the only exception which we can't explain is the source vertex  $f(v, 0)$, which doesn't have any coming edge. However, This first step is established, so it is proved.

To prove the correctness of the multi-shortest path algorithm, we need to establish two key points:


\begin{enumerate}
    \item 1. All optimal solutions are present in the distance table $D$.
    \item 2. All solutions in the distance table $D$ are optimal (when there is no constraint on the size of $D$).
\end{enumerate}

If we can prove that (1) and (2) are correct, implying that they are equivalent, then we can establish the correctness of our algorithm.

Regarding item (1), since the dynamic programming equation considers all edges that link to vertex $v$, we can guarantee that we find all possible temporary solutions, which contain all optimal solutions.

As for item (2), assume that $f(v, \ell)$ is Pareto optimal, and there exists $d_u \in f(u, \ell-1)$ that is not a Pareto optimal solution. Due to the monotonicity feature of the cost function, after $d_u \in f(u, \ell-1)$ is connected with the weight cost $d(u, v)$, it still will not be a Pareto optimal solution. After the pruning step, these worse solutions would be dominated, which means $f(v, \ell)$ will not be the Pareto optimal solution. This leads to the conclusion that for all $d_v \in f(v, \ell)$ to be Pareto optimal, all $f(u, \ell-1)$ for $u \in \text{in}(v)$ and $f(v, \ell-1)$ must be Pareto optimal solutions. In other words, only when the previous iteration contains Pareto optimal solutions can the next iteration still contain all Pareto optimal solutions. The only exception we cannot explain is the source vertex $f(v, 0)$, which does not have any incoming edges. However, this initial step is established, so it is proved.\\

\textbf{Convergence property}\\
If $s \rightsquigarrow u \rightarrow v$ is shortest path in $G$ for some $u,v \in V$ ,and if $u.d = \delta(s,u)$ at any time prior to relaxing $edge(u,v)$, then $v.d = \delta(s,v)$ at all times afterward.\\




==> algorithm/graph.tex <==
Our approach involves handling the minimization of cost for a single edge, which can be analogized to the concept of finding the shortest path. We manage this by maintaining and updating a table to capture the trade-offs among various types of costs. This table is instrumental in recording and managing the interplay of different cost criteria for a given source node $s$ and destination node $v$.

\begin{algorithm}
\caption{Generate Edges and Targets}
\begin{algorithmic}[1]
    \State \textbf{Input} $V$
    \State $E \gets \{\}$
    \For{vertex $u$ in $V$}
        \For{vertex $v$ in $V$}
            \If{is-connected(vertex $u$, vertex $v$)}
                \State $E$.add(make-edge(vertex $u$, vertex $v$))
            \EndIf
        \EndFor
    \EndFor
    \State targets $\gets \{\}$
    \For{vertex $u$ in $V$}
        \If{is-target(vertex $u$)}
            \State targets.add(vertex $u$)
        \EndIf
    \EndFor
    \State \%make vertex-dummy
    \For{vertex $t$ in targets}
        \State $E$.add(make-edge(vertex $t$, vertex-dummy))
        \State \% make the cost of edge zero
    \EndFor
\end{algorithmic}
\end{algorithm}

Firstly, we extract data point from high dimensional data space, and then we build a graph for those data points through k-NN. Initially, an empty set of edges, denoted as $E$, is created, and then iterates through each pair of vertices in the input set $V$, checking if there is a connection between them. If a connection is found, an edge is created between the two vertices and added to the set $E$. Subsequently, the algorithm identifies target vertices by iterating through each vertex in $V$ and checking if it is a target vertex. Target vertices are added to a set called `targets`. In order to address this problem. A dummy vertex is created and we introduce it into to the graph structure. For each target vertex identified, an edge with zero cost is added between the target vertex and the dummy vertex. 

Secondly, user then decides on the properties of target instance - counterfactual. Under what circumstances is it considered a successful flip? Before that, here are some rule your customized cost function need to follow:
Assume s :[0,1]x[0,1] → [0,1], make $\mu_{A \cup B}(X)$ = s[$\mu_A(X) \cup \mu_B(X)$]

\begin{itemize}
    \item [(1)]
    Boundary conditions:\\
    s(1,1) = 1, and s$(\mu_A(X),0)$ = s(0,$\mu_A(X)$) = $\mu_A(X)$
    \item [(2)]
    Monotonicity:\\
    if $\mu_A(X)$<$\mu_c(X)$ and $\mu_B(X)$<$\mu_D(X)$\\
    then $s(\mu_A(X), \mu_B(X)) \leq s(\mu_C(X), \mu_D(X))$
    \item [(3)]
    commutativity:\\
    s($\mu_A(X), \mu_B(X)$) = s($\mu_B(X), \mu_A(X)$)
    \item [(4)]
    Associativity:\\
    s($\mu_A(X), s(\mu_B(X), \mu_C(X)$)) = s(s($\mu_A(X), \mu_B(X)), \mu_C(X)$)
\end{itemize}
For example, taking the maximum value and addition. After all preparatory work is completed, we can start our recourse algorithm.





==> algorithm/multi-criteria.tex <==
\paragraph{Algorithm}
we adapt and modify the Bellman-Ford algorithm which use a dynamic programming approach. The main goal is to handle the minima cost within all considered criteria.

\begin{algorithm}
\caption{Multi-shortest-path}
\begin{algorithmic}[1]
    \Function{Multi-shortest-path}{$G = \{E,V\}, source$}
        \State {\# Initialization}
        \For{each $V$ in $G$}
            \State$D_v \gets \phi$
        \EndFor
        \State$D_{source} \gets \{0\}$
        %\State$t_s \gets$add a terminal point
        
        \State {\# Bellman-Ford algorithm.}
        \For{$i \gets 1$ to $v-1$}
            \For{each $E$}
                (x, y belong to E)
                \State update($D_y, (D_x, T_{xy})$)
            \EndFor
            \State$D_y \gets$dominate($D_y$)
        \EndFor
        \State \Return$D$
    \EndFunction
\end{algorithmic}
\end{algorithm}

\begin{figure}[ht!]
\centering
\includegraphics[width=60mm]{structure.png}
\caption{Schematic diagram for using Use $u$ to relax the distance of $\overline{sv}$ \label{structure}}
\end{figure}

Considering multiple cost criteria, algorithm2 computes the shortest paths from a given source vertex to all other vertices in a graph. The distance list $D_v$ represents the set of target points for reaching vertex $v$ from the source vertex. Initially, all item in $D_v$ are empty except for the source vertex. We set the distance to itself $D_s$ as zero for all cost dimensions. 

Secondly, it employs a modified version of the Bellman-Ford algorithm. During each iteration, it iterates over the vertices excluding the source and conducts a tailored merging process, for each edge $(x, y)$ in the graph, performs an update operation. The update operation extends the $D_y$for the destination vertex $y$ by combining the distance from the source vertex $x$ with the cost of the current edge $(x, y)$ and pruning step. Let $f^\prime (u, \ell - 1) = update(f(u, \ell - 1), d(u, v))$, which means update $D_u$ by connect with edge $\overline{uv}$
\todo{use "update" in pseudo code might be confused with the dp equation}
\begin{equation}
\begin{aligned}
f(v, \ell) = prune_{u \in \text{in}(v)}(\text{concatenate}\left(f^\prime (u, \ell - 1)) ,f(v, \ell - 1)\right)
\end{aligned}
\end{equation}

\textbf {concatenate} 

The concatenate operation is responsible for updating the distance $D$ estimate f(v, $\ell$) for a target vertex v at iteration $\ell$ by combining the distance estimates f(u, $\ell$ - 1) from the source to all vertices u that have an incoming edge to v (denoted by u $\in$ in(v)), with the respective costs d(u, v) of the edges from u to v. The f(u, $\ell$ - 1) represents the distance estimate from the source to the vertex u at the previous iteration $\ell$ - 1. Based on the Bellman-Ford algorithm, the concatenate operation uses the distance estimate f(u, $\ell$ - 1) from the source to u to update or "relax" the cost or distance estimate f(v, $\ell$) for the target vertex v. It considers all possible paths from adjacent vertices to v through u, accumulating the distances along the way.\\

\textbf {prune} 
 
After obtaining the distances through the concatenate operation. The prune operation is employed to refine the distances estimate f(v, $\ell$) for a vertex v at iteration $\ell$ by comparing the trade-offs between the current estimate f(v, $\ell$ - 1) and the newly merged distances from the adjacent vertices u $\in$ in(v). It then iterates through the sorted list, ensures that the distance list remains compact and efficient by retaining only the dominant points that represent the most significant trade-offs in the multi-dimensional space.  


\todo {whether we need to add table size control}
Additionally, if the size of the pruned distance list exceeds a specified limit, the prune function further reduces the list by sampling a fixed number of points at equal intervals, preserving the overall shape of the cost curve while limiting its size. This sampling process helps manage the size of the distance lists and ensures efficiency in subsequent calculations.
% Once all edges have been processed, the algorithm returns the list of distance $D$. These distance capture the trade-offs between different cost criteria and can be used for efficient decision-making in various scenarios, such as transportation or communication networks, where multiple cost factors influence path selection.

\begin{algorithm}
\caption{Backtracking Algorithm}
\begin{algorithmic}[1]
    \Function{backtracking}{$S, T, D$}
        \State paths$\gets$[]
        \For{$u$ belongs to$D_T$}
            \State path$\gets$[]
            \State$v \gets T$
            \While{$v \neq S$}
                \State path.add($u$)
                \State cost$\gets$get edge cost($v, u$)
                \For{each$i$belongs to$D_u$}
                    \If{cost$v ==$cost$u +$cost}
                        \State find parent if cost$v ==$cost$u +$cost
                        \State$v \gets u$
                        \State$u \gets i$
                    \EndIf
                \EndFor
            \EndWhile
            \State paths.add(path)
        \EndFor
        \State \Return paths
    \EndFunction
\end{algorithmic}
\end{algorithm}

The Backtracking Algorithm is used to find paths in a graph from a target vertex back to a source vertex, given certain constraints. The algorithm operates by exploring possible paths starting from each vertex in a set of destination vertices $D_T$, backtracking to the source vertex $S$. For each destination vertex $u$ in the set $D_T$, the algorithm initiates a search for a path by traversing edges backward from $u$ to $S$. It does so by iterative examining edges and their associated costs, identifying the parent vertex that minimizes the total cost to reach $u$ from $S$. This process continues until the source vertex $S$ is reached. The algorithm then records the discovered path and proceeds to explore paths from other destination vertices. Once all possible paths have been explored, the algorithm returns the collected paths. This approach is useful for various applications, including finding optimal routes in transportation networks or identifying dependencies in computational tasks.

==> experiments/adult.tex <==
\subsection{Adult}


    In this study, we introduce a novel method based on multi-cost shortest path algorithms and validate its effectiveness on the Adult dataset. The Adult dataset is Here are the specific steps and methodologies we employed in our experiment.


We started by standardizing the "Adult" dataset to ensure uniformity across various features, allowing for more accurate comparisons. Using a random forest model with 100 trees, then we sorted this standardized dataset and also maintained a non-standardized version for diverse analytical needs. Based on a set of predefined actionable criteria, we established an actionable dataset. During this process, some criteria were set as immutable to reflect real-world conditions. For instance, in the Adult dataset, gender was designated as immutable. From this actionable dataset, we randomly selected 256 instances that met predefined actionable criteria for further analysis. These instances were assessed using a second random forest model to identify the data points with the lowest success probability, indicating areas with the highest challenges.

For data analysis, we created a KNN-graph (k=4) from the standardized dataset and applied our multi-cost shortest path algorithm to explore optimal changes in three key dimensions: education, hours per week, and age. We used the non-standardized data to calculate the shortest paths based on these criteria, aiming to find the most optimized change strategies within these three dimensions. To ensure a realistic application, we designed different cost functions for each criterion. Taking "age" for example, when designing the cost function, it is notable that age can not decrease during the whole recourse process. %As mentioned in Algorithm~\ref{algo:backtracking}, we use Pareto optimal 2 to prune the paths, retaining only a representative set of costs.
    
Figure~\ref{fig:enter-label} visualized the results of the experiment that getting multiple flipped counterfactuals. These four paths, originating from the same starting point where the success probability is the worst, illustrate the diverse impacts caused by Pareto optimal solutions, and all four paths ultimately reach an endpoint where the success probability exceeds 0.75. The introduction of Kernel Density Estimation (KDE) into the algorithm demonstrates a better trade-off with other costs, enhancing the algorithm's ability to navigate through the solution space effectively. To better visualize and understand the patterns in the data, we applied Principal Component Analysis (PCA) for dimension reduction.

%In conclusion, the application of our algorithm on the Adult dataset has demonstrated significant capabilities in addressing complex decision-making scenarios where multiple factors such as age and hours worked per week impact income predictions. Our approach effectively identifies optimal paths for improving individual income predictions by leveraging a multi-criteria framework. This enables a tailored intervention strategy that considers multiple aspects of an individual’s profile.

==> experiments/figures.tex <==



%\begin{figure}
%    \centering
%    \includegraphics[width=0.4\textwidth]{}
%    \includegraphics[width=0.4\textwidth]{experiments/1.pdf}
%    \includegraphics[width=0.4\textwidth]{experiments/2.pdf}

%    \caption{Paths of images transform from 2 to 8}
%\end{figure}




==> experiments/mnist.tex <==
\subsection{MNIST}

In this experiment, we explore the influence of multiple criteria on the MNIST dataset.

The MNIST dataset is a large collection of handwritten digit images, widely utilized for training image processing systems and benchmarking machine learning algorithms.

We commence by extracting a subset from the original MNIST dataset. Subsequently, we construct a K-Nearest Neighbors (KNN) graph using the L2 metric for distance calculation. Leveraging this graph, we introduce two cost criteria: 1) the difference between the labels of the images, and 2) the L2 distance between the images themselves. Furthermore, we employ the max function to update the former cost.

In essence, the aim is to identify the shortest path transition from the source to the target, while adhering to a specific threshold of label difference.

The following table and Figure 2 present the results of our experiment.
\begin{table}[ht]
\centering


\begin{tabular}{|c|l|c|c|}
    \hline
    Image & Path& Cost$_1$& Cost$_2$\\
    \hline
    1 & 2 $\rightarrow$ 4 $\rightarrow$ 4 $\rightarrow$ 6$\rightarrow$ 8 & 2 & 31 \\
    2 & 2 $\rightarrow$3$\rightarrow$ 8 & 5 & 15 \\
    3 & 2 $\rightarrow$ 8 & 6 & 8.7 \\
    \hline
\end{tabular}
\caption{Paths from 2 to 8}
\label{tab:mnist_path}
\end{table}
% We compare our approach with the Fast Approximate Counterfactual Explanations (FACE) method. In FACE, we use Kernel Density Estimation (KDE) as the cost for each edge and apply Dijkstra's algorithm. The resulting images are presented in the figure 3. From this figure, it is evident that the FACE algorithm can only generate a single path.

% By comparing the results of our multi-criteria approach with FACE, we aim to gain insights into the effectiveness of different cost functions in generating counterfactual explanations for the MNIST dataset.

% Our experiments clearly illustrated that while the FACE method is constrained to producing a single transformation path, our multi-cost approach facilitates exploring a wider array of potential transformations. This capacity not only enriches the set of counterfactual explanations available but also enhances the interpretability and adaptability of the model by providing diverse alternatives that meet different criteria.

==> experiments/scalability.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{experiments/scale.pdf}
    \caption{show scalability}
    \label{fig:scalability}
\end{figure}



==> related.tex <==

% In the realm of decision-making, the integration of recourse mechanisms represents a significant advancement, particularly influencing how decisions impact individuals in critical sectors such as finance, healthcare, and education. Originating from the need to enhance the interpretability~\cite{gunning2019xai,arrieta2020explainable,guidotti2018survey} and accountability of machine learning and artificial intelligence models, recourse mechanisms provide individuals a clear pathway to understand and potentially modify the decisions that affect their lives directly. In the financial sector, recourse helps loan applicants understand necessary improvements for a higher likelihood of loan approval~\cite{barocas2017fairness, mukerjee2002multi}. In healthcare, it offers patients explanations and potential lifestyle changes aligned with their treatment plans~\cite{bastani2017interpretability,bertossi2020asp,liang2014deep}. Similarly, in education, recourse aids in analyzing student assessments and admissions, providing insights into academic outcomes, and suggesting avenues for improvement~\cite{fiok2022explainable,khosravi2022explainable}.

% Most algorithms developed for recourse in decision-making are based on gradient methods, which rely on the differentiability of cost functions associated with decision models~\cite{shao2022gradient}. These algorithms typically provide one-hop solutions, offering direct, feasible changes that an individual can make to alter the decision outcome in their favor. This approach, however, assumes that all aspects of the decision-making model are differentiable, which is not always the case.

% Initially developed to make machine learning and AI models more interpretable and accountable, recourse mechanisms face significant challenges, particularly when navigating the high-dimensional space of user attributes. Each attribute acts as a distinct dimension, complicating the identification of optimal recourse paths in real-world scenarios. Traditional recourse algorithms, mainly gradient-based, offer one-hop solutions but often struggle with discrete decisions or thresholds, limiting their applicability and effectiveness. Moreover, these methods lack comprehensive theoretical analysis and rely on approximations, which can compromise their efficacy and transparency. To address these issues, our work aims to push the boundaries of recourse methodologies by proposing innovative solutions for non-differentiable cost functions. This expansion allows for a wider application of recourse strategies, enhancing their ability to handle a variety of decision models that are not amenable to traditional approaches, ultimately providing a more principled foundation for analyzing and implementing recourse in decision-making processes.

% Transitioning from these challenges, contemporary methods such as FACE and GDPR's counterfactual explanations serve as practical implementations that address the issues of interpretability and operational feasibility in high-dimensional spaces.


% Building on these innovations, methods like FACE (Poyiadzi et al. 2020)\cite{poyiadzi2020face} which employs shortest path distances with density-weighted metrics to generate feasible and actionable counterfactual explanations, demonstrate how contemporary recourse mechanisms can integrate more intuitive and natural frameworks for machine learning applications. FACE constructs a graph over the data points using approaches such as KDE, k-NN, or e-graph. By approximating the f-distance using a finite graph over the dataset and incorporating additional feasibility and classifier confidence constraints, FACE provides a natural and intuitive framework for generating meaningful explanations in machine learning applications. Similarly, Automated Decisions and the GDPR (Wachter et al. 2017)\cite{wachter2017counterfactual} discusses counterfactual explanations in the context of GDPR and introduces the foundational ideas that could be extended using shortest path methods to generate actionable insights. This approach aims to generate alternative scenarios related to specific decisions by computing the shortest path, thereby providing an understanding of the logic behind automated decisions while meeting the transparency and interpretability requirements of the GDPR. 

% In the evolving landscape of algorithmic recourse, Feasible Recourse Plan via Diverse Interpolation(Nguyen et al. 2023)~\cite{nguyen2023feasible} proposes a novel approach to generate diverse recourse plans, integrating multiple criteria such as cost, validity, diversity, and adherence to the data manifold, aiming to align with the different preferences of users and the data structure. It emphasizes the construction of diverse prototypes using training data, contributing a comprehensive method to produce insightful recourse plans and data structure-aligned. Additionally, it presents state-of-the-art techniques to generate counterfactual points along the data manifold, enhancing the diversity and distribution understanding of the data. 
% In the context of algorithmic recourse, our approach uniquely emphasizes dynamic pathways for altering decision outcomes of models, focusing on mapping out feasible paths that go beyond mere adjustments of data points. Unlike the methods proposed by FACE and Automated Decisions and the GDPR, which largely center on generating counterfactual explanations using shortest path distances within a graph-based framework or under GDPR compliance, our method delves into the continuous and practical transformations required to achieve favorable outcomes. By emphasizing the entire journey of changes rather than isolated adjustments, our methodology not only integrates the user's actual constraints and possibilities but also aligns with diverse user preferences and data structures as highlighted by Feasible Recourse Plan via Diverse Interpolation. This path-oriented approach offers a holistic and action-oriented solution, providing a broader perspective on recourse actions and ensuring a deeper integration with the practical realities faced by users.

% Our approach is particularly effective in complex scenarios where multiple changes are feasible, and each change impacts the decision in different ways. Our algorithm stands out by handling these multi-criteria cases effectively, ensuring that the recourse provided is not only theoretically optimal but also practically feasible and fair.

% -

In decision-making systems, the integration of recourse mechanisms significantly influences how decisions impact individuals in critical sectors such as finance, healthcare, and education. These mechanisms, designed to enhance the interpretability and accountability of machine learning and AI models, provide individuals a clear pathway to understand and potentially modify decisions affecting their lives ~\cite{gunning2019xai,arrieta2020explainable,guidotti2018survey}. In finance, recourse helps loan applicants understand necessary improvements for higher loan approval chances ~\cite{barocas2017fairness}. In healthcare, it offers patients explanations and potential lifestyle changes aligned with their treatment plans ~\cite{bastani2017interpretability,bertossi2020asp,liang2014deep}. Similarly, in education, recourse aids in analyzing student assessments and admissions, providing insights and improvement suggestions ~\cite{fiok2022explainable,khosravi2022explainable}.

Most algorithms for recourse in decision-making rely on gradient methods, assuming differentiable cost functions associated with decision models ~\cite{shao2022gradient}. These algorithms typically offer one-hop solutions, which are direct changes an individual can make to alter the decision outcome. However, these methods struggle with discrete decisions or thresholds and lack comprehensive theoretical analysis, relying on approximations that compromise efficacy and transparency.

To address these issues, our work proposes innovative solutions for non-differentiable cost functions, expanding the application of recourse strategies. This approach enhances the ability to handle various decision models not amenable to traditional approaches, providing a more principled foundation for analyzing and implementing recourse.

Contemporary methods like FACE (Poyiadzi et al. 2020)\cite{poyiadzi2020face} and GDPR (Wachter et al. 2017)\cite{wachter2017counterfactual}’s counterfactual explanations serve as practical implementations addressing interpretability and operational feasibility in high-dimensional spaces. FACE employs shortest path distances with density-weighted metrics to generate feasible and actionable counterfactual explanations \cite{poyiadzi2020face}. Automated Decisions and the GDPR discuss counterfactual explanations in the GDPR context, introducing foundational ideas extended using shortest path methods for actionable insights (Wachter et al. 2017)\cite{wachter2017counterfactual}.

Building on these innovations, our approach, Feasible Recourse Plan via Diverse Interpolation, proposes a novel method to generate diverse recourse plans, integrating multiple criteria such as cost, validity, diversity, and adherence to the data manifold, Feasible Recourse Plan via Diverse Interpolation(Nguyen et al. 2023)~\cite{nguyen2023feasible}. This method emphasizes constructing diverse prototypes using training data, enhancing the generation of insightful recourse plans and understanding the data structure. Our approach focuses on mapping out feasible paths for altering decision outcomes, integrating user constraints and preferences, and ensuring practical and fair solutions.

==> thebibliography.tex <==
% ---- Bibliography ----
%
% BibTeX users should specify bibliography style 'splncs04'.
% References will then be sorted and formatted in the correct style.
%
% \bibliographystyle{splncs04}
% \bibliography{mybibliography}
%
\begin{thebibliography}{8}

\bibitem{mothilal2020explaining}
Mothilal, R.K., Sharma, A., Tan, C.: Explaining machine learning classifiers through diverse counterfactual explanations. In: Proceedings of the 2020 Conference on Fairness, Accountability, and Transparency, pp. 607--617 (2020)

\bibitem{gabow1984scaling}
Gabow, H.N., Bentley, J.L., Tarjan, R.E.: Scaling and related techniques for geometry problems. In: Proceedings of the Sixteenth Annual ACM Symposium on Theory of Computing, pp. 135--143 (1984)

\bibitem{preparata2012computational}
Preparata, F.P., Shamos, M.I.: Computational Geometry: An Introduction. 2nd edn. Springer Science \& Business Media, (2012)

\bibitem{karlsson1988scanline}
Karlsson, R.G., Overmars, M.H.: Scanline algorithms on a grid. BIT Numerical Mathematics \textbf{28}, 227--241 (1988)

\bibitem{bellman1958routing}
Bellman, R.: On a routing problem. Quarterly of Applied Mathematics \textbf{16}(1), 87--90 (1958)

\bibitem{agarwal2005geometric}
Agarwal, P.K., Har-Peled, S., Varadarajan, K.R., et al.: Geometric approximation via coresets. Combinatorial and Computational Geometry \textbf{52}(1), 1--30 (2005)

\bibitem{haussler1986epsilon}
Haussler, D., Welzl, E.: Epsilon-nets and simplex range queries. In: Proceedings of the Second Annual Symposium on Computational Geometry, pp. 61--71 (1986)

\bibitem{jiang2011free}
Jiang, P., Chen, Y.: Free lunches on the discrete Lipschitz class. Theoretical Computer Science \textbf{412}(17), 1614--1628 (2011)

\bibitem{daston2021objectivity}
Daston, L., Galison, P.: Objectivity. Princeton University Press, (2021)

\bibitem{chen2020simple}
Chen, T., Kornblith, S., Norouzi, M., Hinton, G.: A simple framework for contrastive learning of visual representations. In: International Conference on Machine Learning, pp. 1597--1607. PMLR (2020)

\bibitem{lundberg2018consistent}
Lundberg, S.M., Erion, G.G., Lee, S.I.: Consistent individualized feature attribution for tree ensembles. arXiv preprint arXiv:1802.03888 (2018)

\bibitem{lundberg2018explainable}
Lundberg, S.M., et al.: Explainable machine-learning predictions for the prevention of hypoxaemia during surgery. Nature Biomedical Engineering \textbf{2}(10), 749--760 (2018)

\bibitem{tang2022perception}
Tang, Y., et al.: Perception and navigation in autonomous systems in the era of learning: A survey. IEEE Transactions on Neural Networks and Learning Systems (2022)

\bibitem{kingma2013auto}
Kingma, D.P., Welling, M.: Auto-encoding variational bayes. arXiv preprint arXiv:1312.6114 (2013)

\bibitem{doersch2016tutorial}
Doersch, C.: Tutorial on variational autoencoders. arXiv preprint arXiv:1606.05908 (2016)

\bibitem{fang2020independent}
Fang, S., Zhu, Q.: Independent Gaussian distributions minimize the Kullback-Leibler (KL) divergence from independent Gaussian distributions. arXiv preprint arXiv:2011.02560 (2020)

\bibitem{zhai2018autoencoder}
Zhai, J., Zhang, S., Chen, J., He, Q.: Autoencoder and its various variants. In: 2018 IEEE International Conference on Systems, Man, and Cybernetics (SMC), pp. 415--419. IEEE (2018)

\bibitem{monti2019fake}
Monti, F., Frasca, F., Eynard, D., Mannion, D., Bronstein, M.M.: Fake news detection on social media using geometric deep learning. arXiv preprint arXiv:1902.06673 (2019)

\bibitem{wang2018deep}
Wang, C., Han, D., Liu, Q., Luo, S.: A deep learning approach for credit scoring of peer-to-peer lending using attention mechanism LSTM. IEEE Access \textbf{7}, 2161--2168 (2018)

\bibitem{kim2023help}
Kim, S.S.Y., Watkins, E.A., Russakovsky, O., Fong, R., Monroy-Hernández, A.: "Help Me Help the AI": Understanding how explainability can support human-AI interaction. In: Proceedings of the 2023 CHI Conference on Human Factors in Computing Systems, pp. 1--17 (2023)

\bibitem{turay2022toward}
Turay, T., Vladimirova, T.: Toward performing image classification and object detection with convolutional neural networks in autonomous driving systems: A survey. IEEE Access \textbf{10}, 14076--14119 (2022)

\bibitem{danilevsky2020survey}
Danilevsky, M., et al.: A survey of the state of explainable AI for natural language processing. arXiv preprint arXiv:2010.00711 (2020)

\bibitem{wu2022graph}
Wu, S., et al.: Graph neural networks in recommender systems: a survey. ACM Computing Surveys \textbf{55}(5), 1--37 (2022)

\bibitem{wang2021deep}
Wang, M., Deng, W.: Deep face recognition: A survey. Neurocomputing \textbf{429}, 215--244 (2021)

\bibitem{zhao2019object}
Zhao, Z.Q., Zheng, P., Xu, S., Wu, X.: Object detection with deep learning: A review. IEEE Transactions on Neural Networks and Learning Systems \textbf{30}(11), 3212--3232 (2019)

\bibitem{otter2020survey}
Otter, D.W., Medina, J.R., Kalita, J.K.: A survey of the usages of deep learning for natural language processing. IEEE Transactions on Neural Networks and Learning Systems \textbf{32}(2), 604--624 (2020)

\bibitem{voynov2020unsupervised}
Voynov, A., Babenko, A.: Unsupervised discovery of interpretable directions in the GAN latent space. In: International Conference on Machine Learning, pp. 9786--9796. PMLR (2020)

\bibitem{goodfellow2014generative}
Goodfellow, I., et al.: Generative adversarial nets. Advances in Neural Information Processing Systems \textbf{27} (2014)

\bibitem{ho2020denoising}
Ho, J., Jain, A., Abbeel, P.: Denoising diffusion probabilistic models. Advances in Neural Information Processing Systems \textbf{33}, 6840--6851 (2020)

\bibitem{baldi2012autoencoders}
Baldi, P.: Autoencoders, unsupervised learning, and deep architectures. In: Proceedings of ICML Workshop on Unsupervised and Transfer Learning, pp. 37--49. JMLR Workshop and Conference Proceedings (2012)

\bibitem{luo2022understanding}
Luo, C.: Understanding diffusion models: A unified perspective. arXiv preprint arXiv:2208.11970 (2022)

\bibitem{bank2023autoencoders}
Bank, D., Koenigstein, N., Giryes, R.: Autoencoders. Machine Learning for Data Science Handbook: Data Mining and Knowledge Discovery Handbook, pp. 353--374. Springer (2023)

\bibitem{blei2017variational}
Blei, D.M., Kucukelbir, A., McAuliffe, J.D.: Variational inference: A review for statisticians. Journal of the American Statistical Association \textbf{112}(518), 859--877 (2017)

\bibitem{yang2017understanding}
Yang, X.: Understanding the variational lower bound. Variational lower bound, ELBO, hard attention \textbf{22}, 1--4 (2017)

\bibitem{bishop1998latent}
Bishop, C.M.: Latent variable models. In: Learning in Graphical Models, pp. 371--403. Springer, Heidelberg (1998)

\bibitem{ramesh2022hierarchical}
Ramesh, A., Dhariwal, P., Nichol, A., Chu, C., Chen, M.: Hierarchical text-conditional image generation with clip latents. arXiv preprint arXiv:2204.06125 \textbf{1}(2), 3 (2022)

\bibitem{wu2023brief}
Wu, T., He, S., Liu, J., Sun, S., Liu, K., Han, Q.-L., Tang, Y.: A brief overview of ChatGPT: The history, status quo and potential future development. IEEE/CAA Journal of Automatica Sinica \textbf{10}(5), 1122--1136 (2023)

\bibitem{koh2017understanding}
Koh, P.W., Liang, P.: Understanding black-box predictions via influence functions. In: International Conference on Machine Learning, pp. 1885--1894. PMLR (2017)

\bibitem{sundararajan2020many}
Sundararajan, M., Najmi, A.: The many Shapley values for model explanation. In: International Conference on Machine Learning, pp. 9269--9278. PMLR (2020)

\bibitem{winter2002shapley}
Winter, E.: The Shapley value. Handbook of Game Theory with Economic Applications \textbf{3}, 2025--2054. Elsevier (2002)

\bibitem{hart1989shapley}
Hart, S.: Shapley value. In: Game Theory, pp. 210--216. Springer, Heidelberg (1989)

\bibitem{roth1988introduction}
Roth, A.E.: Introduction to the Shapley value. The Shapley Value, pp. 1--27. University of Cambridge Press, Cambridge (1988)

\bibitem{shapley1953value}
Shapley, L.S.: A value for n-person games. Princeton University Press, Princeton (1953)

\bibitem{pouyanfar2018survey}
Pouyanfar, S., Sadiq, S., Yan, Y., Tian, H., Tao, Y., Reyes, M.P., Shyu, M.L., Chen, S.C., Iyengar, S.S.: A survey on deep learning: Algorithms, techniques, and applications. ACM Computing Surveys (CSUR) \textbf{51}(5), 1--36 (2018)

\bibitem{slack2020fooling}
Slack, D., Hilgard, S., Jia, E., Singh, S., Lakkaraju, H.: Fooling lime and shap: Adversarial attacks on post hoc explanation methods. In: AAAI/ACM Conference on AI, Ethics, and Society, pp. 180--186. (2020)

\bibitem{zhang2019should}
Zhang, Y., Song, K., Sun, Y., Tan, S., Udell, M.: "Why Should You Trust My Explanation?" Understanding Uncertainty in LIME Explanations. arXiv preprint arXiv:1904.12991 (2019)

\bibitem{ray2023chatgpt}
Ray, P.P.: ChatGPT: A comprehensive review on background, applications, key challenges, bias, ethics, limitations and future scope. Internet of Things and Cyber-Physical Systems. Elsevier (2023)

\bibitem{castelvecchi2016can}
Castelvecchi, D.: Can we open the black box of AI? Nature News \textbf{538}(7623), 20 (2016)

\bibitem{guidotti2018survey}
Guidotti, R., Monreale, A., Ruggieri, S., Turini, F., Giannotti, F., Pedreschi, D.: A survey of methods for explaining black box models. ACM Computing Surveys (CSUR) \textbf{51}(5), 1--42 (2018)

\bibitem{yu2023antifake}
Yu, Z., Zhai, S., Zhang, N.: AntiFake: Using Adversarial Audio to Prevent Unauthorized Speech Synthesis. In: ACM SIGSAC Conference on Computer and Communications Security, pp. 460--474. (2023)

\bibitem{arrieta2020explainable}
Arrieta, A.B., Díaz-Rodríguez, N., Del Ser, J., Bennetot, A., Tabik, S., Barbado, A., García, S., Gil-López, S., Molina, D., Benjamins, R., others: Explainable Artificial Intelligence (XAI): Concepts, taxonomies, opportunities and challenges toward responsible AI. Information Fusion \textbf{58}, 82--115 (2020)

\bibitem{stepin2021survey}
Stepin, I., Alonso, J.M., Catala, A., Pereira-Fariña, M.: A survey of contrastive and counterfactual explanation generation methods for explainable artificial intelligence. IEEE Access \textbf{9}, 11974--12001 (2021)

\bibitem{verma2020counterfactual}
Verma, S., Boonsanong, V., Hoang, M., Hines, K.E., Dickerson, J.P., Shah, C.: Counterfactual explanations and algorithmic recourses for machine learning: A review. arXiv preprint arXiv:2010.10596 (2020)

\bibitem{goyal2019counterfactual}
Goyal, Y., Wu, Z., Ernst, J., Batra, D., Parikh, D., Lee, S.: Counterfactual visual explanations. In: International Conference on Machine Learning, pp. 2376--2384. PMLR (2019)

\bibitem{van2008visualizing}
Van der Maaten, L., Hinton, G.: Visualizing data using t-SNE. Journal of Machine Learning Research \textbf{9}(11) (2008)

\bibitem{dong2019variable}
Dong, J., Rudin, C.: Variable importance clouds: A way to explore variable importance for the set of good models. arXiv preprint arXiv:1901.03209 (2019)

\bibitem{shwartz2017opening}
Shwartz-Ziv, R., Tishby, N.: Opening the black box of deep neural networks via information. arXiv preprint arXiv:1703.00810 (2017)

\bibitem{mackiewicz1993principal}
Maćkiewicz, A., Ratajczak, W.: Principal components analysis (PCA). Computers \& Geosciences \textbf{19}(3), 303--342 (1993)

\bibitem{ribeiro2018anchors}
Ribeiro, M.T., Singh, S., Guestrin, C.: Anchors: High-precision model-agnostic explanations. In: AAAI conference on artificial intelligence \textbf{32}(1) (2018)

\bibitem{lundberg2017unified}
Lundberg, S.M., Lee, S.I.: A unified approach to interpreting model predictions. Advances in Neural Information Processing Systems \textbf{30} (2017)

\bibitem{dwivedi2023explainable}
Dwivedi, R., Dave, D., Naik, H., Singhal, S., Omer, R., Patel, P., Qian, B., Wen, Z., Shah, T., Morgan, G., others: Explainable AI (XAI): Core ideas, techniques, and solutions. ACM Computing Surveys \textbf{55}(9), 1--33 (2023)

\bibitem{angelov2020towards}
Angelov, P., Soares, E.: Towards explainable deep neural networks (xDNN). Neural Networks \textbf{130}, 185--194 (2020)

\bibitem{ribeiro2016should}
Ribeiro, M.T., Singh, S., Guestrin, C.: "Why should i trust you?" Explaining the predictions of any classifier. In: ACM SIGKDD International Conference on Knowledge Discovery and Data Mining, pp. 1135--1144. (2016)

\bibitem{miller2023explainable}
Miller, T.: Explainable ai is dead, long live explainable ai! hypothesis-driven decision support. arXiv preprint arXiv:2302.12389 (2023)

\bibitem{jacovi2023trends}
Jacovi, A.: Trends in Explainable AI (XAI) Literature. arXiv preprint arXiv:2301.05433 (2023)

\bibitem{wang2022disentangled}
Wang, X., Chen, H., Tang, S., Wu, Z., Zhu, W.: Disentangled representation learning. arXiv preprint arXiv:2211.11695 (2022)

\bibitem{alzubaidi2021review}
Alzubaidi, L., Zhang, J., Humaidi, A.J., Al-Dujaili, A., Duan, Y., Al-Shamma, O., Santamaría, J., Fadhel, M.A., Al-Amidie, M., Farhan, L.: Review of deep learning: Concepts, CNN architectures, challenges, applications, future directions. Journal of Big Data \textbf{8}, 1--74 (2021)

\bibitem{gunning2019xai}
Gunning, D., Stefik, M., Choi, J., Miller, T., Stumpf, S., Yang, G.Z.: XAI—Explainable artificial intelligence. Science Robotics \textbf{4}(37), eaay7120 (2019)


\end{thebibliography}

